Perturbation CheckLists for Evaluating NLG Evaluation Metrics

Natural Language Generation (NLG) evaluation is a multifaceted task requiring assessment of multiple desirable criteria, e.g., fluency, coherency, coverage, relevance, adequacy, overall quality, etc. Across existing datasets for 6 NLG tasks, we observe that the human evaluation scores on these multiple criteria are often not correlated. For example, there is a very low correlation between human scores on fluency and data coverage for the task of structured data to text generation. This suggests that the current recipe of proposing new automatic evaluation metrics for NLG by showing that they correlate well with scores assigned by humans for a single criteria (overall quality) alone is inadequate. Indeed, our extensive study involving 25 automatic evaluation metrics across 6 different tasks and 18 different evaluation criteria shows that there is no single metric which correlates well with human scores on all desirable criteria, for most NLG tasks. Given this situation, we propose CheckLists for better design and evaluation of automatic metrics. We design templates which target a specific criteria (e.g., coverage) and perturb the output such that the quality gets affected only along this specific criteria (e.g., the coverage drops). We show that existing evaluation metrics are not robust against even such simple perturbations and disagree with scores assigned by humans to the perturbed output. The proposed templates thus allow for a fine-grained assessment of automatic evaluation metrics exposing their limitations and will facilitate better design, analysis and evaluation of such metrics.

==> additional_details.tex <==
In particular, the preprocessing of the sentences370involves  a  combination  of  tokenization,  part-of-371speech tagging, named entity recognition, etc. The372targeted part of the sentence is then modified ei-373ther by leveraging simple string manipulation func-374tions  or  by  masking  and  generating  the  words/375phrases using the predictions by RoBERTa (Liu376et al., 2019).  For example, the application of the377template for ‘dropping stop words’ involves the378tokenization of the sentence using the NLTK word379tokenizer as the first step. The list of tokens is com-380pared with the set of stopwords provided by NLTK381to filter out the stop words from the list of tokens.382The modified sentence is then reconstructed using383the string join function by iterating over the tokens384in the modified list.   Similarly,  for the template385of ‘changing the attributes’ in case of image cap-386tioning, the sentence is first tokenized, then the ad-387jectives are identified using part-of-speech tagging388(again a functionality provided by NLTK). The list389of ‘related words’ (i.e., hyponyms of hypernyms390or ‘sibling words’) are obtained using WordNet391framework.  Unless the list returns empty, one of392the entries in the list is used to replace the origi-393nal adjective.  In order to ‘change question to an394assertive statement’, the question words (such as395who, what, why, when, etc) are replaced with a396‘mask’ token and the ‘?’ character at the end is re-397placed with ‘.’ using string replace function. This398modified sentence is fed to RoBERTa model which399generates different predictions to be used in place400of the ‘mask’ token. One of the suggested words401is  used  to  form  the  modified  assertive  sentence.402(Additional checks are made to ignore any bad sug-403gestiongs for this task such as question words /stop404word suggestion

==> as_metrics_results.tex <==
\begin{table*}[]
\resizebox{1.1\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
Perturbation &
  Criteria &
  BLEU-1  &
  BLEU-4  &
  METEOR &
  ROUGE-L &
  EAvg &
  GM &
  VE &
  CIDEr &
  BERTscore &
  WMDo &
  BLEURT &
  ChrF++ \\ \hline
\cellcolor[HTML]{ECF4FF}Remove punctuation &
  fluency &
  0.8853 &
  0.8023 &
  \cellcolor[HTML]{FFCE93}0.5994 &
  0.8771 &
  0.9902 &
  0.9745 &
  0.9519 &
  7.7029 &
  0.9822 &
  0.212 &
  0.779 &
  93 \\ \hline
\cellcolor[HTML]{ECF4FF}Spelling mistake/typos &
  fluency &
  0.9377 &
  0.8724 &
  \cellcolor[HTML]{FFCE93}0.5913 &
  0.9237 &
  0.9871 &
  0.9766 &
  0.9127 &
  8.238 &
  0.9747 &
  0.168 &
  0.06 &
  96.02 \\ \hline
\cellcolor[HTML]{ECF4FF}Missing stopwords &
  fluency &
  0.4285 &
  0.102 &
  0.3556 &
  0.5607 &
  \cellcolor[HTML]{FFCCC9}0.9024 &
  \cellcolor[HTML]{FFCCC9}0.9201 &
  \cellcolor[HTML]{FFCCC9}0.8583 &
  1.3488 &
  \cellcolor[HTML]{FFCCC9}0.9112 &
  0.264 &
  -0.606 &
  54.6 \\ \hline
\cellcolor[HTML]{ECF4FF}Jumbling words &
  fluency &
  \cellcolor[HTML]{FFCCC9}0.824 &
  0.0101 &
  0.4021 &
  0.321 &
  \cellcolor[HTML]{FFCCC9}1 &
  \cellcolor[HTML]{FFCCC9}1 &
  \cellcolor[HTML]{FFCCC9}0.9992 &
  1.775 &
  \cellcolor[HTML]{FFCCC9}0.8566 &
  0.189 &
  -1 &
  53.23 \\ \hline
\cellcolor[HTML]{B9F7B9}contractions * &
  informativeness &
  0.9308 &
  0.8799 &
  \cellcolor[HTML]{FFCE93}0.6303 &
  0.9173 &
  0.9968 &
  0.991 &
  0.9745 &
  8.3296 &
  0.9984 &
  0.139 &
  0.843 &
  95.6 \\ \hline
\cellcolor[HTML]{B9F7B9}Expansions * &
  informativeness &
  0.9265 &
  0.8719 &
  \cellcolor[HTML]{FFCE93}0.6187 &
  0.9373 &
  0.9982 &
  0.9923 &
  0.9776 &
  8.5513 &
  0.9969 &
  0.125 &
  0.84 &
  96.1 \\ \hline
Reordering sentences &
  flow / coherence &
  1 &
  0.955 &
  0.6703 &
  0.6188 &
  1 &
  1 &
  1 &
  9.511 &
  0.9704 &
  0.173 &
   &
   \\ \hline
\cellcolor[HTML]{B9F7B9}Negating statements &
  informativeness &
  \cellcolor[HTML]{FFCCC9}0.9229 &
  \cellcolor[HTML]{FFCCC9}0.8607 &
  \cellcolor[HTML]{FFCCC9}0.6186 &
  \cellcolor[HTML]{FFCCC9}0.9347 &
  \cellcolor[HTML]{FFCCC9}0.9879 &
  \cellcolor[HTML]{FFCCC9}0.9752 &
  \cellcolor[HTML]{FFCCC9}0.9558 &
  \cellcolor[HTML]{FFCCC9}8.318 &
  \cellcolor[HTML]{FFCCC9}0.9815 &
  \cellcolor[HTML]{FFCCC9}0.19 &
  \cellcolor[HTML]{FFFC9E}0.34 &
  \cellcolor[HTML]{FFCCC9}93.85 \\ \hline
\cellcolor[HTML]{B9F7B9}Synonyms * &
  informativeness &
  0.781 &
  0.6426 &
  0.7059 &
  0.8094 &
  0.9915 &
  0.9111 &
  0.972 &
  5.6512 &
  0.9774 &
  0.172 &
   &
  90.5 \\ \hline
\cellcolor[HTML]{B9F7B9}Using antonyms &
  informativeness &
  \cellcolor[HTML]{FFCCC9}0.7894 &
  \cellcolor[HTML]{FFCCC9}0.6647 &
  \cellcolor[HTML]{FFCCC9}0.5907 &
  \cellcolor[HTML]{FFCCC9}0.8184 &
  \cellcolor[HTML]{FFCCC9}0.9949 &
  \cellcolor[HTML]{FFCCC9}0.98 &
  \cellcolor[HTML]{FFCCC9}0.9405 &
  \cellcolor[HTML]{FFCCC9}5.9313 &
  \cellcolor[HTML]{FFCCC9}0.9764 &
  \cellcolor[HTML]{FFCCC9}0.172 &
  \cellcolor[HTML]{FFCCC9}0.602 &
  \cellcolor[HTML]{FFCCC9}91.59 \\ \hline
  \cellcolor[HTML]{B9F7B9}num2words * &
  informativeness &
   &
   &
   &
   &
   &
   &
   &
   &
  0.9765 &
  0.169 &
  0.714 &
  91.73 \\ \hline
\cellcolor[HTML]{B9F7B9}Replacing with hyponyms &
  informativeness &
  \cellcolor[HTML]{FFCCC9}0.7543 &
  \cellcolor[HTML]{FFCCC9}0.5784 &
  \cellcolor[HTML]{FFCCC9}0.5307 &
  \cellcolor[HTML]{FFCCC9}0.7853 &
  \cellcolor[HTML]{FFCCC9}0.9846 &
  \cellcolor[HTML]{FFCCC9}0.9517 &
  \cellcolor[HTML]{FFCCC9}0.8469 &
  \cellcolor[HTML]{FFCCC9}5.0305 &
  0.9699 &
  0.166 &
  \cellcolor[HTML]{FFCE93}0.476 &
  83.45 \\ \hline
\cellcolor[HTML]{B9F7B9}Replacing 30-40\% content &
  informativeness &
  \cellcolor[HTML]{FFCCC9}0.6717 &
  0.4565 &
  0.4325 &
  \cellcolor[HTML]{FFCCC9}0.6927 &
  \cellcolor[HTML]{FFCCC9}0.9677 &
  \cellcolor[HTML]{FFCCC9}0.9161 &
  \cellcolor[HTML]{FFCCC9}0.7869 &
  3.9738 &
  \cellcolor[HTML]{FFCCC9}0.9483 &
  \cellcolor[HTML]{FFCCC9}0.176 &
  0.07 &
  71.9 \\ \hline
Alternate reference &
   &
  0.2872 &
  0.0655 &
  0.1713 &
  0.2467 &
  0.9025 &
  0.7625 &
  0.5354 &
  0.4781 &
  0.9015 &
   &
   &
   \\ \hline
\end{tabular}%
}
\caption{Performance of metrics on perturbations for Abstractive Summarization}
\label{tab:as_metrics}
\end{table*}
\begin{figure*}
    \centering
    \includegraphics[scale=0.4]{tempp.png}
    \caption{Heat map of Divergence of metric scores from human averages}
    \label{fig:div_as_heatmap}
\end{figure*}
\begin{figure*}
    \centering
    \includegraphics[scale=0.4]{temp.png}
    \caption{Heat map of Divergence of metric scores from human averages}
    \label{fig:div_as_heatmap1}
\end{figure*}


==> correlation_plots.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.7\textwidth]{imgs/dg_scatter.png}
    \caption{Scatter plots for correlation between dialogue criteria \scriptsize{(a small random noise is added to the data points to avoid overlaps)}}
    \label{fig:DG_corrs}
\end{figure*}

==> first_example_table.tex <==
\begin{table*}[]
\begin{tabular}{|L{7.5cm}L{8cm}|}
\hline
Original sentence                                                             & James Cameron is the director of Titanic \\ \hline
\rowcolor[HTML]{DAE8FC} 
Dropping stop words affects fluency but does not miss much of the information & James Cameron is director Titanic        \\ \hline
\rowcolor[HTML]{CBCEFB} 
Changing Named entities does not affect fluency but affects adequacy          & Kate Winslet is the director of Titanic  \\ \hline
\end{tabular}
\end{table*}

==> metrics.tex <==
\begin{table*}[!t]
\resizebox{\textwidth}{!}{%
\begin{tabular}{|C{1cm}|L{4.5cm}|L{12.3cm}|}
\hline
\multicolumn{3}{|c|}{\textbf{Task-agnostic metrics}}                                                                                                                                                                     \\ \hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{\parbox[c]{2.5cm}{\centering {\scriptsize(word / character)} n-gram based }}}    & BLEU-N \cite{bleu}                & checks for overlap of $n$-grams (for $n=1..N$) between reference and hypothesis to compute precision scores along with a brevity penalty term                                                                \\ \cline{2-3} 
                                 & METEOR \cite{meteor}              & matches unigrams based on overlap of surface forms, stemmed words, synonymous words, and paraphrases.                                               \\ \cline{2-3} 
                                 & ROUGE-L  \cite{rouge}         & uses longest common subsequence matching between reference and hypothesis                                                                                                           \\ \cline{2-3} %
                                & CIDEr  \cite{DBLP:conf/cvpr/VedantamZP15_CIDEr}   &  weighs n-grams using TF-IDF (term frequency and inverse document frequency) and computes the cosine similarity of such weight vectors of the reference and candidate \\ \cline{2-3}
                                 & chrF++  \cite{DBLP:conf/wmt/Popovic17_chrFpp}     & computes the F-score using the precision and recall of character n-gram matches along with word-level unigrams and bigrams                                                                    \\ \hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{\parbox[c]{3.5cm}{\centering embedding based}}} & Greedy Matching(GM) \cite{greedymatch}    & Greedy matching (GM): greedily matches embeddings of tokens based on cosine similarity                                                              \\ \cline{2-3} 
                                 & {\small Embedding average (EA) \cite{landauer1997solution_vector_averaging1} } & computes cosine similarity of the average of all token embeddings between reference and hypothesis                          \\ \cline{2-3} 
                                 & Vector Extrema (VE) \cite{vectorextrema}   &the most extreme value along each dimension considering all token embeddings is used to construct final vectors                \\ \cline{2-3} 
                                  & SMS \cite{DBLP:conf/acl/ClarkCS19_sms} &  automatic metric that evaluate text in a continuous
                                    space using word and sentence embeddings.            \\ \cline{2-3}
                                 & WMDo   \cite{chow-etal-2019-WMDO}     &  optimally matches the various token embeddings, allowing partial mappings and many-to-many mappings                                        \\ \hline
\multirow{3}{1cm}{BERT-based/ trained }                      & BERTscore \cite{DBLP:conf/iclr/ZhangKWWA20_BERTscore}             & computes cosine similarity using BERT embeddings and aggregates the greedily matched scores to define an F-score                         \\ \cline{2-3} 
 & MoverScore \cite{DBLP:conf/emnlp/ZhaoPLGME19_MoverScore} & computes distance between BERT embeddings of words and n-grams, allowing partial mappings %
 \\ \cline{2-3} 
\multicolumn{1}{|l|}{}           & BLEURT   \cite{DBLP:conf/acl/SellamDP20_bleurt}        & a trained metric that uses weights learnt from signals based on other metrics: BLEU, ROUGE, BERTscore, etc.         \\  \cline{2-3}
 & GRUEN &  reference less metric that  utilizes a BERT-based model and a class of syntactic, semantic, and contextual features to examine the fluency, redundancy, focus and coherence of the text.
\\ \hline
\hline
\multicolumn{3}{|c|}{\textbf{Task-specific metrics} (All of these are trained metrics except SPICE)}                                                                                                                                                                     \\ \hline
\multirow{2}{*}{AS}      & SUPERT \cite{DBLP:conf/acl/GaoZE20_supert}          & a reference less metrics which rates the quality of a summary by measuring its semantic similarity with a pseudo reference summary generated by selecting salient sentences from the source document using contextualized embeddings                                          \\ \cline{2-3}
& BLANC \cite{DBLP:journals/corr/abs-2002-09836_blanc}    &  a reference less metric that scores a summary based on the performance boost gained by a pretrained language model with access to the summary while carrying out a language understanding tasks on the source text document   \\ \hline
QG        & Q-metrics  \cite{DBLP:conf/emnlp/NemaK18_qbleu}       & metrics which incorporate an answerability score along with n-gram metrics that is based on weights learnt from human evaluation data      \\ \hline
\multirow{4}{*}{DG}              & ADEM   \cite{DBLP:conf/acl/LoweNSABP17ADEM}    &  an hierarchical RNN that is trained to score the generated dialogue response given the context and a candidate response                        \\ \cline{2-3} 
                                 & RUBER  \cite{DBLP:conf/aaai/TaoMZY18ruber}   & scores responses using both vector extrema (along with a reference response) and a bidirectional GRU (along with the context)                \\ \cline{2-3} 
                                 & MaUDe  \cite{DBLP:conf/acl/SinhaPWLHP20_maude}   & unreferenced metric which only scores using the context / history of the conversation                \\ \cline{2-3} 
                                 & DEB   \cite{DBLP:journals/tacl/SaiMAK20_DDpp}     & a BERT-based model that is pretrained on large-scale dialogue specific data takes context and generated response as input to provide the score \\ \hline
\multirow{3}{*}{IC}      & SPICE \cite{DBLP:conf/eccv/AndersonFJG16_SPICE}          &                                               \\ \cline{2-3}
 & TIGEr \cite{DBLP:conf/emnlp/JiangHZWZGDG19_TIGEr}          &         \\ \cline{2-3}
& VilBERT    &   \\ \hline
D2T & PARENT \cite{DBLP:conf/acl/DhingraFPCDC19_parent} & scores the generated text by computing F-measure using both the reference and the data. \\ \hline
\end{tabular}
}
\caption{Existing automatic evaluation metrics considered in our work for various NLG tasks}
\label{tab:metrics_description}
\end{table*}

==> supple.tex <==
\input{supplementary_examples_table}


\section{A few detailed examples to illustrate the implementation of the perturbation templates}
We mainly work with the official github repository\footnote{https://github.com/marcotcr/checklist} of the checklist paper. The implementation involves preprocessing with the help of tokenization, POS tagging, NER recognition, etc. Synonyms, antonyms, etc are obtained with the help of WordNet framework. Additionally, the masked language model of RoBERTa is used to mask and predict replacements for the targeted words. For example, the application of the template for `dropping stop words' involves the tokenization of the sentence using the NLTK word tokenizer as the first step. The list of tokens is compared with the set of stopwords provided by NLTK to filter out the stop words from the list of tokens. The modified sentence is then reconstructed using the string join function by iterating over the tokens in the modified list. Similarly, for the template of `changing the attributes' in case of image captioning, the sentence is first tokenized, then the adjectives are identified using part-of-speech tagging (again a functionality provided by NLTK). The list of `related words' (i.e., hyponyms of hypernyms or `sibling words') are obtained using WordNet framework. Unless the list returns empty, one of the entries in the list is used to replace the original adjective. In order to `change question to an assertive statement', the question words (such as who, what, why, when, etc) are replaced with a `mask' token and the `?' character at the end is replaced with `.' using string replace function. This modified sentence is then fed to RoBERTa model which generates different predictions to be used in place of the `{mask}' token. One of the suggested words is used to form the modified assertive sentence.

Note that some of the perturbations cannot be applied to every sentence in the dataset. For example, the template of ``changing names'' cannot be applied if there are no named entities in a particular sentence. We hence shortlist only the successfully modified samples from the dataset for analysing the metrics' performance on each perturbation. 

==> supplementary_examples_table.tex <==
\section{Perturbation Templates for various criteria (with examples)}
\begin{table*}[!t]
\centering %
\resizebox{1\textwidth}{!}{
\rowcolors{1}{}{lightgray!50}
\begin{tabular}{l L{2cm} L{4cm} L{7.5cm} L{7.5cm}} %
\hline\hline %
\textbf{Task} & \textbf{Criteria} & \textbf{Perturbation} & \textbf{Unmodified sentence} & \textbf{Perturbed sentence} \\ %
\hline \hline%



 \cellcolor{white}   &\cellcolor{white}  &Misplaced/missing punctuation&Could you let me know if I can meet him now or later\colorbox{color}{?}& Could you let me know\colorbox{lightred}{,} if I can meet him now or later\colorbox{lightred}{.}\\
 \cellcolor{white}   &\cellcolor{white}& Jumbling word order & We \colorbox{color}{play} badminton every evening. & We badminton every evening play. \\
    \cellcolor{white}   &\cellcolor{white} & Inconsistent subject-verb agreement   & He \colorbox{color}{doesn't} know how to bake. & He \colorbox{lightred} {don't} know how to bake.\\
    \cellcolor{white}   &\cellcolor{white} &Dropping words (such as prepositions/articles, etc)& \colorbox{color}{The} bank \colorbox{color}{is} willing to approve the loan. & Bank willing to approve the loan. \\
    \multirow{-8}{1.4em}{\cellcolor{white}All tasks} &  \multirow{-8}{*}{\cellcolor{white}Fluency}  &Spelling errors&Make the most of every opportunity presented to you.&Make the most of \colorbox{lightred}{evry} opportunity presented to you.\\
    \hline

    \cellcolor{white}   &\cellcolor{white}    &Dropping out words or phrases &I \colorbox{color}{was being} followed. & I followed. \\ %
    \cellcolor{white}   &\cellcolor{white} &Adding extra wrong information& This book is so inspiring. & This book is so inspiring,\colorbox{lightred} {I forgot}. \\ 
    \cellcolor{white}   &\cellcolor{white} &Negation / antonyms&It \colorbox{color}{will rain} on Monday.&It will \colorbox{lightred}{not} rain on Monday.\\
    \multirow{-7}{1.4em}{\cellcolor{white}MT} & \multirow{-7}{*}{\cellcolor{white}Adequacy}  &Repeat phrases &My relatives are in town.&My relatives are in town, \colorbox{lightred}{my relatives}.\\
    \hline


\cellcolor{white} & \cellcolor{white}  
    &Dropping words& Here is the \colorbox{color}{no parking} sign. & Here is the sign.\\ %
    \cellcolor{white}   &\cellcolor{white} &Negation and antonyms& This book is so \colorbox{color}{inspiring}. & This book is so \colorbox{lightred}{uninspiring}. \\
    \cellcolor{white} &\multirow{-4}{4em}{\cellcolor{white}Informa-tiveness} &Use hyponyms to create misinformation& The girl my \colorbox{color}{brother} Andy met through MySpace turned out to be completely made up . & The girl my \colorbox{lightred}{friend} Andy met through MySpace turned out to be completely made up. \\ 
    \hhline{~----}\hhline{~}
    \cellcolor{white} & \cellcolor{white}Flow / coherence & Reorder sentences & The pandemic was spreading uncontrollably. Vaccines are being developed and tested rapidly.& Vaccines are being developed and tested rapidly. \colorbox{lightred}{The pandemic was spreading uncontrollably.}\\
    \hhline{~----}\hhline{~}
    \cellcolor{white} &\cellcolor{white} Non-Redundancy & Repeat sentences& My relatives are in town. &My relatives are in town. \colorbox{lightred}{My relatives in town.}\\
    \hhline{~----}\hhline{~}
\multirow{-9}{*}{\cellcolor{white}AS}  &\cellcolor{white}Referential clarity& Replace nouns by pronouns& \colorbox{color}{The pandemic} was spreading uncontrollably. \colorbox{color}{Vaccines} are being developed rapidly.&\colorbox{lightred}{It} was spreading uncontrollably. \colorbox{lightred}{They} are being developed rapidly.\\
    \hline

\cellcolor{white} & \cellcolor{white} 
    &Change question word& \colorbox{color}{When} was he born? &\colorbox{lightred}{What} was he born? \\ %
    \cellcolor{white} & \cellcolor{white}  &Drop question word& \colorbox{color}{When} was he born ? & Was he born?\\
    \cellcolor{white} & \cellcolor{white}  &Change question to assertive statement & Who is the director of Titanic? & \colorbox{lightred}{The director of Titanic is James Cameron.}\\
    \cellcolor{white} & \multirow{-5}{4em}{\cellcolor{white}Answera-bility}   &Drop NLTK stop words&Who \colorbox{color}{was not a} world leader&Who world leader?\\
    \hhline{~----}\hhline{~}
    \cellcolor{white} & \cellcolor{white}  &Mask a few words and predict&How could Tesla run \colorbox{color}{the experiments}?&How could Tesla run to \colorbox{lightred}{the beach}?\\
 \multirow{-9}{1.4em}{\cellcolor{white}QG}    & \multirow{-4}{4em}{\cellcolor{white}Relevance} &Perturb named entities, nouns, verbs& Why did \colorbox{color}{Mary} go to the \colorbox{color}{school}? & Why did \colorbox{lightred}{Raj} go to the \colorbox{lightred}{market}? \\%\cline {1-5} 
 \hline

\cellcolor{white} & \cellcolor{white}
    &{\small Negate a previous statement by same speaker}& Bot: I enjoy having your daughter in my class. User: I'm glad to hear that. & I \colorbox{lightred}{don't} enjoy having your daughter in my class.\\ %
    \cellcolor{white} & \multirow{-3}{4em}{\cellcolor{white}Making sense} &Add extra non-sensible text & Do you know where Dr. XYZ lives? & Yes, \colorbox{lightred}{my father is my grandmother's father} \\
    \hhline{~----}\hhline{~}
    \cellcolor{white} & \cellcolor{white}
    & Repeat previous utterances  & Do you know Dr.XYZ?& \colorbox{lightred}{Do you know where Dr. XYZ lives?}\\
    \cellcolor{white} & \multirow{-3}{4em}{\cellcolor{white}Avoid repetition} & Repeat phrases & I like ice creams& I like ice creams, \colorbox{lightred}{ice creams}\\
    \hhline{~----}\hhline{~}
    \cellcolor{white} & \cellcolor{white}Listening & Replace with "Can you repeat?" & I need to book a taxi & \colorbox{lightred}{I'm sorry, can you repeat?}\\
    \hhline{~----}\hhline{~}
    \multirow{-11}{*}{\cellcolor{white}DG} & \cellcolor{white}Relevance & Map random responses & I am \colorbox{color}{new to coding}. & I am \colorbox{lightred}{scared of snakes}.\\
    \hline
    
\cellcolor{white} & \cellcolor{white} & Change the order of objects & The \colorbox{color}{man} is standing in front of a \colorbox{color}{tree} & The tree is standing in front of man \\
    \cellcolor{white} & \cellcolor{white}
    & Change gender  &  Two \colorbox{color}{girls} are playing with a doll & Two \colorbox{lightred}{boys} are playing with a doll\\
    \cellcolor{white} & \multirow{-3}{3em}{\cellcolor{white}Correctness} & Change attributes  &  A \colorbox{color}{small} boy playing with a \colorbox{color}{red} ball & A \colorbox{lightred}{tall} boy playing with a \colorbox{lightred}{green} ball\\
    \hhline{~----}\hhline{~}
    \cellcolor{white} & \cellcolor{white}
    & Drop objects/noun  & A small \colorbox{color}{boy} playing with a red \colorbox{color}{ball} &  A small playing with a red \\
    \multirow{-6}{*}{\cellcolor{white}IC} & \multirow{-2}{4em}{\cellcolor{white}Thoroughness} & Repeat (append) object & A lady riding a horse. & A lady riding a horse \colorbox{lightred}{and a lady}.\\
    \hline

    \cellcolor{white} & \cellcolor{white} & Use hyponyms & Beethoven was a German \colorbox{color}{musician} & Beethoven was a German \colorbox{lightred}{architect} \\
    \cellcolor{white} & \cellcolor{white}
    & Change numbers  &  The cricketer was born in \colorbox{color}{1990}. & The cricketer was born in \colorbox{lightred}{1950}.\\
    \cellcolor{white} & \multirow{-3}{4em}{\cellcolor{white}Correctness} & Negation / antonyms &  The author of Harry Potter is J.K Rowling & The author of Harry Potter is \colorbox{lightred}{not} J.K Rowling.\\
    \hhline{~----}\hhline{~}
    \cellcolor{white} & \cellcolor{white}
    & Drop phrases  & A small boy playing with a \colorbox{color}{red ball} &  A small boy playing with a \\
    \cellcolor{white} & \multirow{-3}{4em}{\cellcolor{white}Data Coverage} & Repeat phrases & Beethoven was a German musician & Beethoven was a German musician \colorbox{lightred}{and German musician}.\\
    \hhline{~----}\hhline{~}
    \cellcolor{white} & \cellcolor{white}
    & Random text& Beethoven was a German musician & \colorbox{lightred}{The cricketer was born in 1990.}\\ %
    \multirow{-10}{*}{\cellcolor{white}D2T}& \cellcolor{white}Relevance & Perturb names & \colorbox{color}{Phillips} was a child prodigy. & \colorbox{lightred}{James} was a child prodigy.\\
    \hline



\cellcolor{white} & \cellcolor{white}
    &Replace with synonyms&The mangoes are \colorbox{color}{delicious}. & The mangoes are \colorbox{lightred}{tasty}.\\ %
    \cellcolor{white} & \cellcolor{white}&Contractions&We \colorbox{color}{are} going to embark on an adventure. & \colorbox{lightred}{We're} going to embark on an adventure.\\ 
    \cellcolor{white} & \cellcolor{white}&Expansions&There \colorbox{color}{weren't} any clear winners of the contest&There \colorbox{lightred}{were not} any clear winners of the contest.\\
    \multirow{-5}{1.4em}{\cellcolor{white}All tasks}   & \multirow{-5}{*}{\cellcolor{white}Invariance} &Numerals to words&Aron Ralston who was trapped for \colorbox{color}{127} hours.&Aron Ralston who was trapped for \colorbox{lightred}{one hundred twenty seven} hours.\\
    \cline{1-4}
\hline
\end{tabular}}
\caption{Perturbation templates targeting various criteria with examples. The blue highlights indicate the portions of the original sentence affected by the perturbation template. The red highlights indicate the changes in the modified sentence.}
\label{table:examples_suppl} %
\end{table*}
